Improved bounds for polylogarithmic graph distances in scale-free percolation and related models

In this paper, we study graph distances in the geometric random graph models scale-free percolation SFP, geometric inhomogeneous random graphs GIRG, and hyperbolic random graphs HRG. Despite the wide success of the models, the parameter regime in which graph distances are polylogarithmic is poorly understood. We provide new and improved lower bounds. In a certain portion of the parameter regime, those match the known upper bounds. Compared to the best previous lower bounds by Hao and Heydenreich, our result has several advantages: it gives matching bounds for a larger range of parameters, thus settling the question for a larger portion of the parameter space. It strictly improves the lower bounds by Hao and Heydenreich for all parameters settings in which those bounds were not tight. It gives tail bounds on the probability of having short paths, which imply shape theorems for the $k$-neighbourhood of a vertex whenever our lower bounds are tight, and tight bounds for the size of this $k$-neighbourhood. And last but not least, our proof is much simpler and not much longer than two pages, and we demonstrate that it generalizes well by showing that the same technique also works for first passage percolation.

==> couplings.tex <==




As mentioned earlier, our recursive proof of the lower bound(s) only works for sufficiently small percolation parameter $\percparam$. However, it turns out that we can couple an instance of \LRP \:or \SFP \:with arbitrary $\percparam$ to one with sufficiently small $\percparam$, paying a corresponding overhead factor in shortest distances. We show how this is achieved in this section.

\subsection{Coupling in LRP}
Let us first focus on the simple case of \LRP \:. We will use $\LRPbig$ to refer to the instance of \LRP \:with arbitrary $\percparam$ and $\LRPsmall$ to refer to that with a sufficiently small $\percparam$. Similarly, we will use $\percparambig$ and $\percparamsmall$ to distinguish between the two percolation parameters. We will always think of $\percparamsmall$ as small enough for the recursion proof to work. The idea is to in some way \textit{expand} $\mathbb{Z}^d$ for $\LRPsmall$, as if one zoomed in their view of it. That is, we select some (integer) factor $\blowupparam$ and associate each point in $\LRPbig$ with a box of $\blowupparam^d$ points of $\LRPsmall$. For a given point/vertex $u$, let $\boxofpoints{u}$ be the corresponding set of points/vertices in the associated box. Then, the coupling works as follows. Depending on the edge realisations of $\LRPsmall$, we insert an edge in $\LRPbig$ between two vertices $u, v$ if and only if an edge exists in $\LRPsmall$ connecting a pair of vertices $u_s, v_s$ with $u_s \in \boxofpoints{u}$ and $v_s \in \boxofpoints{v}$. Figure \ref{fig:coupling-LRP} illustrates this procedure.

\begin{figure}[ht]
\centering
\begin{tikzpicture}[scale=0.75, every node/.style={scale=0.75}]
    \foreach \x in {0,2,4}
        \foreach \y in {0,2,4}
            \coordinate (big-\x-\y) at (\x,\y);
    
    \foreach \x in {0,2,4}
        \foreach \y in {0,2,4}
            \filldraw[fill=blue!20!white, draw=black] (big-\x-\y) circle (0.1);
    
    \node[above left] at (big-0-4) {$u$};
    \node[below right] at (big-4-0) {$v$};
    
    \draw[thick, blue, bend right=30] (big-0-4) to (big-4-0);
    
    \def\smallgrid{0.5}
    \begin{scope}[shift={(6,-1)},scale=\smallgrid]
        \foreach \x in {2,...,10}
            \foreach \y in {2,...,10}
                \filldraw[fill=red!20!white, draw=black] (\x,\y) circle (0.1/\smallgrid);
        
        \coordinate (small-u) at (1.5,7.5);
        \coordinate (small-v) at (7.5,1.5);
        \draw[thick, black] (small-u) rectangle ++(3,3);
        \draw[thick, black] (small-v) rectangle ++(3,3);
        
        
        \node[above right] at (0, 10) {$\boxofpoints{u}$};
        \node[below left] at (12, 1.5) {$\boxofpoints{v}$};
        
        \filldraw[fill=red!60!white, draw=black] (3,9) circle (0.1/\smallgrid);
        \filldraw[fill=red!60!white, draw=black] (9,3) circle (0.1/\smallgrid);
        \draw[thick, red, bend left=30] (3,9) to (9,3);
    \end{scope}
\end{tikzpicture}
\caption{Illustration of the coupling between $\LRPbig$ and $\LRPsmall$ focusing on two vertices. Nearest-neighbor edges are omitted for clarity. Here, $\blowupparam = 3$ is chosen, hence each vertex in $\LRPbig$ is replaced with $\blowupparam^d = 3^2 = 9$ vertices in $\LRPsmall$. Note that an edge exists (in blue) between 
$u$ and $v$ in $\LRPbig$ because one exists (in red) between a pair of vertices from $\boxofpoints{u}$ and $\boxofpoints{v}$ in $\LRPsmall$.}
\label{fig:coupling-LRP}
\end{figure}

To be completely precise, the corresponding graph that arises through this coupling is not exactly $\LRPbig$, but instead some stochastic graph model which dominates $\LRPbig$, from now on named $\LRPcoupling(\blowupparam)$. That is, each edge is present in this model with a probability that is larger than that of $\LRPbig$ (including nearest neighbor edges, which can be thought of as having probability 1). This is sufficient for our purpose of obtaining a lower bound on graph distances. That being said, let us now lower bound the probability of connection in $\LRPcoupling(r)$.

\begin{lemma}\label{lem:blowupprobbound}
Let $u, v$ be two vertices in $\LRPcoupling(\blowupparam)$. The edge $\{u, v\}$ is present with probability at least $\probconnection{c\percparamsmall \blowupparam^{d(2 - \alphaparam)}}$ and independently of all other edges, for some absolute constant $c$.
\end{lemma}

\begin{proof}
    It suffices to show that $\mathbb{P}[\text{the edge $\{u, v\}$ is missing}] \le \probnotconnection{c\percparamsmall \blowupparam^{d(2 - \alphaparam)}}$. To see this, note that for at least a constant fraction of the pairs between $\boxofpoints{u}$ and $\boxofpoints{v}$ it is true that their distance in $\LRPsmall$ is at most $\blowupparam|u - v|$. Therefore, we have:

    \[\mathbb{P}[\text{the edge $\{u, v\}$ is missing}] \le \left(\mathbb{P}[\text{an edge $\{u', v'\}$ with } |u' - v'| \le \blowupparam|u - v| \text{ is missing in $\LRPsmall$}]\right)^{c \blowupparam^{2d}}\]
    \[\le \probnotconnection{c \blowupparam^{2d} \percparamsmall \blowupparam^{-d\alphaparam}} = \probnotconnection{c\percparamsmall \blowupparam^{d(2 - \alphaparam)}}\]
\end{proof}

Now, with Lemma \ref{lem:blowupprobbound}, we can link the probability of a short path in $\LRPbig$ with that of an appropriately (but not much) longer path in $\LRPsmall$.

\begin{lemma}\label{lem:shortpathsmaintained}
Let $u, v$ be two vertices in $\LRPbig$. Then,
    \[\mathbb{P}[\graphdist{u}{v} \le x \text{ in } \LRPbig] \le \mathbb{P}[\graphdist{u'}{v'} \le c_{\percparambig} x \text{ in } \LRPsmall]\]
where $|u' - v'| = \Omega(\blowupparam|u - v|)$, and $c_{\percparambig}$ and $\blowupparam$ only depend on parameters of the model.
\end{lemma}

\begin{proof}
    Note that for large enough $\blowupparam$ (so that the factor $c\percparamsmall \blowupparam^{d(2 - \alphaparam)}$ in Lemma \ref{lem:blowupprobbound} is at least $\percparambig$), $\LRPbig$ is dominated by $\LRPcoupling(\blowupparam)$. Also note that this is possible because $\alphaparam < 2$. Hence, it suffices to show the claim for the latter. For this, one can see that a path of graph-theoretic length $x$ between $u$ and $v$ implies the existence of a path with graph-theoretic distance at most $3d\blowupparam x$ between some $u'$ and $v'$ in $\LRPsmall$, with $u' \in \boxofpoints{u}$ and $v' \in \boxofpoints{v}$.  This is because one can always walk between any two vertices in $\boxofpoints{w}$ for any $w$ using at most $d\blowupparam$ steps and also because any edge $\{w_1, w_2\}$ used in the path in $\LRPcoupling(\blowupparam)$ implies that an edge exists between some pair of vertices from \boxofpoints{w_1} and \boxofpoints{w_2}. Therefore, a path is constructed by taking the cross-box edges and stitching them together with walks within the boxes. We choose as $u', v'$ the pair which maximizes the Euclidean distance among all pairs from \boxofpoints{u} and \boxofpoints{v}, therefore $|u' - v'| = \Omega(\blowupparam|u - v|)$.
\end{proof}

    
\subsection{Coupling in SFP}
Let us reuse the naming conventions established for \LRP\:but add the power law exponent $\tauparam$ as a superscript. Crucially, note that the percolation parameter needs to be small enough \textit{with respect to} $\tauparam$ for the recursive proof to go through (the integration constants are affected). Thus, $\SFPsmall{\tauparam}$ will be assumed to have such a small enough percolation parameter. The situation is quite similar in \SFP. In fact, the coupling is exactly the same. That is, we still simply observe what happens in $\SFPsmall{\tauparam}$ and add an edge in $\SFPcoupling{\tauparam}(r)$ if and only if there is an edge between the corresponding boxes. Note that we only sample weights for $\SFPsmall{\tauparam}$. The new objective here will be to argue about the ``weight" (whatever that will be) distribution of $\SFPcoupling{\tauparam}(r)$ and somehow show that it dominates the weight distribution of $\SFPbig{\tauparam}$. 

It turns out that relating $\SFPcoupling{\tauparam}(r)$ to $\SFPbig{\tauparam}$ is not that easy. What we do instead is choose a \textit{smaller} $\tauparam'$ and compare $\SFPcoupling{\tauparam'}(r)$ to $\SFPbig{\tauparam}$. Intuitively, since we will be in some way averaging weights drawn in $\SFPsmall{\tauparam'}$, the decrease in the power law exponent is necessary to ensure that we still have high chances of getting a high average (via the maximum sample), compared to a single sample with exponent $\tauparam$. 

Now, to get a sense of what the weights in $\SFPcoupling{\tauparam'}(r)$ will be, let us show a lower bound on the probability of connection, akin to that shown in Lemma \ref{lem:blowupprobbound}.

\begin{lemma}\label{lem:blowupboundSFP}
    Let $u, v$ be two vertices in $\SFPcoupling{\tauparam'}(\blowupparam)$ and $\percparambig$ be a ``goal" percolation parameter. Conditioned on the complete set of weights for each point in $\mathbb{Z}^d$ (in $\SFPsmall{\tauparam'}$), the edge $\{u, v\}$ is present with probability at least
    \[1 - e^{-\percparambig |u - v|^{-d\alphaparam} (W_u)^{\alphaparam} (W_v)^{\alphaparam}}\]
    where
    \[W_x = c\frac{\left(\sum\limits_{x' \in \boxofpoints{x}}(w_{x'})^{\alphaparam}\right)^{\frac{1}{\alphaparam}}}{r^{\frac{d}{2}}}, x \in \{u, v\}\]
    and independently of all other edges, for some $c$ not depending on $\blowupparam$.
\end{lemma}

\begin{proof}
    The proof is very similar to that of Lemma \ref{lem:blowupprobbound}. However, instead of a constant fraction of pairs between $\boxofpoints{u}$ and $\boxofpoints{v}$, we consider all their pairs and instead bound each of their distances by $3dr|u - v|$. This bound can be seen by the triangle inequality (by going through the centers of the boxes to connect $u'$ and $v'$) and noting that $|u-v| \ge 1$. The bound then follows by algebraic manipulation.
\end{proof}

Now, in light of Lemma \ref{lem:blowupboundSFP}, we only need to show that $W$ as defined above stochastically dominates any power law distribution with parameter $\tauparam$ for large enough $\blowupparam$, since we have pattern matched the connection probability accordingly to compare it to that of $\SFPbig{\tauparam}$. In the following, we will use $\powerlaw{\tauparam}$ to refer to the latter distribution.

Essentially, we are looking at the $\alphaparam$-norm of $n$ samples of the original distribution and then dividing by $\sqrt{n}$ (and some constant). Here, $n = \blowupparam^d$. We will consider two extreme ways in which this distribution can yield high values. The first and simpler one comes from the fact that we take many samples, all of which have a value of at least 1.

\begin{prop}
    $\mathbb{P}[W \ge c n^{\frac{1}{\alphaparam} - \frac{1}{2}}] = 1$, where $c$ is as in Lemma \ref{lem:blowupboundSFP} and $n = \blowupparam^d$. In particular, $\mathbb{P}[W \ge x] \ge \mathbb{P}[\powerlaw{\tauparam} \ge x]$ for all $x \le c n^{\frac{1}{\alphaparam} - \frac{1}{2}}$.
\end{prop}
\begin{proof}
Since deterministically each $w_x \ge 1$, we have $W \ge c\frac{\left(\sum\limits_{x' \in \boxofpoints{x}}1\right)^{\frac{1}{\alphaparam}}}{n^{\frac{1}{2}}} = c n^{\frac{1}{\alphaparam} - \frac{1}{2}}$. Therefore this happens with probability 1.
\end{proof}


The second way in which $W$ can get high values is through its maximum sample. 

\begin{prop} \label{pr:tauprime}
    There exists a constant $c'$ such that $\mathbb{P}[W \ge x] \ge \mathbb{P}[\powerlaw{\tauparam} \ge x]$ for all $x \ge c'n^{\frac{\tauparam' - 3}{2(\tauparam - \tauparam')}}$, where $\tauparam'$ is the power law exponent used in the definition of $W$.
\end{prop}
\begin{proof}
    Let $w_{max}$ refer to the maximum value observed from the $n$ samples taken to generate $W$. Below, $c$ is as in Lemma \ref{lem:blowupboundSFP}. There exists a $c_1$ such that for large enough $x$:

    \[\mathbb{P}[W \le x] \le \mathbb{P}\left[w_{max} \le \frac{n^{1/2}}{c}x\right] = \left(\mathbb{P}\left[\powerlaw{\tauparam'} \le \frac{n^{1/2}}{c}x\right]\right)^{n}\]
    \[\le \left(1 - c_1\left(\frac{n^{1/2}}{c}x\right)^{1 - \tauparam'}\right)^{n} \le e^{-n^{1 - \frac{\tauparam' - 1}{2}}c^{\tauparam' - 1}c_1x^{1-\tauparam'}}\]

    Moreover, there exists a $c_2$ such that for large enough $x$ we have:
    \[\mathbb{P}[\powerlaw{\tauparam} \le x] \ge 1 - c_2x^{1-\tauparam} \ge e^{-2c_2x^{1-\tauparam}}\]

    Combining the two bounds, we see that $\mathbb{P}[W \le x] \le \mathbb{P}[\powerlaw{\tauparam} \le x]$ whenever:
    \[\frac{n^{1 - \frac{\tauparam' - 1}{2}}c^{\tauparam' - 1}c_1x^{1-\tauparam'}}{2c_2x^{1-\tauparam}} \ge 1 \iff x \ge c' n^{\frac{\tauparam' - 3}{2(\tauparam - \tauparam')}}\]

    for some $c'$ which only depends on $\tauparam, \tauparam', c, c_1, c_2$.
\end{proof}

Now, combining the two previous propositions, we can choose a small enough $\tauparam'$ so that domination is guaranteed throughout the whole range of possible $x$ values. Specifically, we only need to set $\tauparam'$ such that:
\[\frac{\tauparam' - 3}{2(\tauparam - \tauparam')} < \frac{1}{\alphaparam} - \frac{1}{2} \iff \tauparam' < \tauparam \left(1 - \frac{\alphaparam}{2}\right) + 3\frac{\alphaparam}{2}\] 
Note that there exist values of $\tauparam' > 3$ that satisfy this inequality, as $\tauparam > 3$. Once such a $\tauparam'$ is fixed, domination is ensured for $n$ (i.e. $\blowupparam^d$) large enough.


\begin{lemma}\label{lem:shortpathsmaintainedSFP}
Let $u, v$ be two vertices in $\SFPbig{\tauparam}$. Then for a suitable $\tauparam'$,
    \[\mathbb{P}[\graphdist{u}{v} \le x \text{ in } \SFPbig{\tauparam}] \le \mathbb{P}[\graphdist{u'}{v'} \le c_{\percparambig} x \text{ in } \SFPsmall{\tauparam'}]\]
where $|u' - v'| = \Omega(\blowupparam|u - v|)$, and $c_{\percparambig}$ and $\blowupparam$ only depend on parameters of the model.
\end{lemma}
\begin{proof}
    The proof is entirely symmetrical to that of Lemma \ref{lem:shortpathsmaintained}. One simply needs to set an appropriate $\tauparam'$ as in Proposition \ref{pr:tauprime} and then take $\blowupparam$ large enough so that the weight distribution of $\SFPcoupling{\tauparam'}$ dominates that of $\SFPbig{\tauparam}$.
\end{proof}

\subsection{Decreasing the $\alphaparam$ parameter.}
Another requirement for the recursive proof to work is that we have $\alphaparam < \tauparam - 2$. This is not an essential requirement, but rather an artifact of the proof strategy. However, we will show here that one can assume that $\alphaparam$ is small enough so that this condition holds by changing $\percparam$ accordingly (note that $\tauparam - 2 > 1$).
\begin{lemma}
    Let $\alphaparam$ and $\percparam$ be the long-range and percolation parameters of some instance of \SFP. Fix the weights of all vertices and let $p_{u, v}$ refer to the probability that arbitrary vertices $u$ and $v$ are connected by an edge. Then, $p_{u, v} \le \min\{1, \percparam^{\frac{\alphaparam'}{\alphaparam}}w_u^{\alphaparam'} w_v^{\alphaparam'} |u-v|^{-d{\alphaparam'}}\}$. But that does not help unfortunately.
\end{lemma}


==> lrp_proof.tex <==

\section{Lower Bounds for Graph Distances in LRP}\label{sec:LRP}

In this section, we prove \Cref{thm:lowerboundLRP}. Our contribution here is the significantly simplified proof compared to the original one in \cite{Biskup_2004}. Furthermore, it illustrates the techniques used in the next section for SFP. 

As mentioned before, our proof works by expressing the probability that the shortest path between $x, y$ has at most $k$ edges recursively, which allows us to inductively prove a bound on the lower tail of the distribution of $\dg{x}{y}$. However -- in its pure form -- this inductive proof only works for a sufficiently small constant $\lambda$ controlling the connection probability. But remarkably, it turns out that only showing this is in fact enough to prove our result for all $\lambda$, which we establish by creating a coupling between an instance of LRP with small $\lambda$ and an instance of LRP with arbitrary $\lambda$ in which the length of a shortest path increases only by a constant. We start with the first part of the argument, and later establish the coupling in \Cref{sec:couplings}.

\begin{lemma}\label{lem:lrpmainproof}
    Consider LRP with $\alpha \in (1, 2)$ and sufficiently small $\lambda$, and fix some arbitrarily small $\varepsilon > 0$. Let $\Delta' = \Delta + \varepsilon$. Then for all $\varepsilon > 0, k \ge 1$, $k \in \mathbb{N}$, we have \begin{align*}
        \Pr{ \dg{x}{y} \le k } \le |x-y|^{-\alpha d} e^{\alpha d k^{1 / \Delta'} }.
    \end{align*}
\end{lemma} \begin{proof}
    We proceed by induction over $k$. The base case ($k = 1$) follows immediately as \begin{align*}
        \Pr{ \dg{x}{y} \le 1 } = \pLRP = \min\{ 1 , \lambda |x - y|^{-\alpha d} \} \le |x-y|^{-\alpha d} e^{\alpha d k^{1 / \Delta'} }
    \end{align*} for sufficiently small $\lambda$. For general $k$, we use a recursive relation to bound $\Pr{ \dg{x}{y} \le k }$. The idea is as follows. If there is a path of length $\le k$ from $x$ to $y$, then at least one edge $\{ u, v \}$ on that path has a (geometric) length of at least $\frac{|x - y|}{k}$, and moreover $\dg{x}{u} + \dg{v}{y} \le k - 1$. So for some $0 \le \ell \le k - 1$, there are paths $P_{x, u}$ of length $\ell$, $P_{u, v}$ of length $1$, and $P_{v, y}$ of length $k - \ell - 1$, while all these paths are edge-disjoint. Hence -- if we view LRP as a product probability space over all the potential edges -- the event \begin{align*}
        \mathcal{E}_{k, \ell}^{(u,v)} \coloneqq \{ \dg{x}{u} \le \ell \} \disjointoccurence \{ u \sim v\} \disjointoccurence \{ \dg{v}{y} \le k - \ell - 1 \}
    \end{align*} must occur.
    Thus, we can bound $\Pr{ \dg{x}{y} \le k }$ by summing over all possible $u,v \in \mathbb{Z}^d$ with $|u - v| \ge |x-y|/k$ and over all possible values of $\ell$. To this end, denote by $S \subseteq \mathbb{Z}^d \times \mathbb{Z}^d$ the set of all tuples $(u, v)$ such that $|u - v| \ge |x - y| / k$, and observe that \begin{align*}
        \Pr{ \dg{x}{y} \le k } &\le \sum_{\ell = 0}^{k-1} \sum_{(u, v) \in S} \Pr{ \{ \dg{x}{u} \le \ell \} \disjointoccurence \{ u \sim v\} \disjointoccurence \{ \dg{v}{y} \le k - \ell - 1 \} } \\
        &\le \sum_{\ell = 0}^{k-1} \sum_{(u, v) \in S} \Pr{ \dg{x}{u} \le \ell } \Pr{ u \sim v} \Pr{ \dg{v}{y} \le k - \ell - 1 }  \\
    \end{align*} by the BK-inequality (\Cref{cor:BK}). We now use the induction hypothesis and replace the sum over all pairs $(u,v) \in S$ by two integrals over the distances $r_u \coloneqq |x - u|$ and $r_v \coloneqq |v - y|$. We further replace $\Pr{ u \sim v} \le \lambda (|x  - y|/k)^{-d\alpha}$ since $u, v$ have distance at least $|x  - y|/k$.
    With this, there is a constant $C_1$ (that depends on the model parameters) such that 
    \fontsize{10}{12}\selectfont
    \begin{align*}
        &\Pr{ \dg{x}{y} \le k } \\
        &\hspace{.4cm}\le C_1 \lambda \left( \frac{|x - y|}{k} \right)^{-\alpha d} \sum_{\ell = 0}^{k-1} \int_{1}^{\infty} \int_{1}^{\infty} r_u^{d-1} \min\left\{1 ,  \frac{e^{\alpha d\ell^{1/\Delta'}}}{r_u^{\alpha d}}  \right\} r_v^{d-1} \min\left\{1 ,  \frac{e^{\alpha d\left(k - \ell - 1\right)^{1/\Delta'}}}{r_v^{\alpha d}}  \right\} \d r_u \d r_v \\
        &\hspace{.4cm} = C_1 \lambda \left( \frac{|x - y|}{k} \right)^{-\alpha d} \sum_{\ell = 0}^{k-1} \underbrace{\left( \int_{1}^{\infty} r_u^{d-1} \min\left\{1 ,  \frac{e^{\alpha d\ell^{1/\Delta'}}}{r_u^{\alpha d}}  \right\} \d r_u \right)}_{I_u}  \underbrace{\left(\int_{1}^{\infty} r_v^{d-1} \min\left\{1 ,  \frac{e^{\alpha d\left(k - \ell - 1 \right)^{1/\Delta'}}}{r_v^{\alpha d}}  \right\} \d r_v \right)}_{I_v}
    \end{align*}
    \normalsize
    \todo[inline]{Well technically it can't be that $\ell = 0$ or $\ell = k-1$ because we're using $r_u, r_v \geq 1$, and if $\ell = 0$ or $\ell = k-1$ then either $u$ and $x$ coincide or $v$ and $y$ coincide, so probably we need to consider this term separately.}
    We proceed by bounding $I_u, I_v$ and obtain \begin{align*}
        I_u = \int_{1}^{\hat{r}} r^{d-1} \d r + \int_{\hat{r}}^\infty r^{d - \alpha d - 1} e^{\alpha d\ell^{1/\Delta'}} \d r
    \end{align*} where $\hat{r} = e^{\ell^{1/\Delta'}}$ is the point at which the minimum changes. Solving the integrals yields that there is a constant $C_2 > 0$ such that \begin{align*}
        I_u &\le \frac{C_2}{2} \left( \hat{r}^d + e^{\alpha d\ell^{1/\Delta'}} \hat{r}^{d(1 - \alpha)} \right) = C_2 e^{d\ell^{1/\Delta'}}.
    \end{align*}
    Similarly, we obtain $I_v = C_3 e^{ d(k-\ell-1)^{1/\Delta'}}$ for some constant $C_3 > 0$. Thus, in total \begin{align*}
        \Pr{ \dg{x}{y} \le k } &\le \lambda C \left( \frac{|x - y|}{k} \right)^{-\alpha d} \sum_{\ell = 0}^{k-1} \exp\left( d\ell^{1/\Delta'} + d(k - \ell - 1)^{1/\Delta'} \right).
    \end{align*} Now, for all $0 \le \ell \le k-1$, we have \begin{align*}
        \ell^{1/\Delta'} + (k - \ell - 1)^{1/\Delta'} \le 2\left( k/2 \right)^{1/\Delta'}.
    \end{align*} Hence, if we replace the sum by $k$ times its maximum, we obtain \begin{align*}
        \Pr{ \dg{x}{y} \le k } &\le \lambda C \left( \frac{|x - y|}{k} \right)^{-\alpha d} k \exp\left( 2d\left( k/2 \right)^{1/\Delta'} \right).
    \end{align*} 
    Now choose $\varepsilon' > 0$ such that $\frac{1}{\Delta'} = \frac{1}{\Delta} + \varepsilon'$. \KP{Something's off here, in the statement of the lemma it says $\Delta' > \Delta$, whereas here it seems $\frac{1}{\Delta'} > \frac{1}{\Delta}$ --- these can't both be true, and it should be the latter, right?} Since $\Delta = 1/\log_2(2 / \alpha)$, we have $2^{-1/\Delta} = \alpha / 2$, so \begin{align*}
        2(k/2)^{1/\Delta'} = \alpha k^{1/\Delta'} 2^{-\varepsilon'}.
    \end{align*} Therefore, \begin{align*}
        \Pr{ \dg{x}{y} \le k } &\le \lambda C |x - y|^{-\alpha d} k^{1 + \alpha d} \exp\left( \alpha d k^{1/\Delta'}2^{-\varepsilon'} \right)\\
        &= |x - y|^{-\alpha d} \exp\left( \alpha d k^{1/\Delta'} \right) \cdot \lambda \underbrace{C k^{1 + \alpha d} \exp\left( \alpha d k^{1/\Delta'}(2^{-\varepsilon'} - 1) \right)}_{\coloneqq f(k)}.
    \end{align*} Now, since $\varepsilon' > 0$, we have that $\lim_{k \rightarrow \infty} f(k) = 0$ so in particular, there is some $k_0$ such that for all $k \ge k_0$, we have $f(k) \le 1$. Thus, if we choose any $\lambda \le (\max_{1 \le k \le k_0} f(k))^{-1}$, we can conclude that \begin{align*}
        \Pr{ \dg{x}{y} \le k } &\le |x - y|^{-\alpha d} \exp\left( \alpha d k^{1/\Delta'} \right)
    \end{align*} for all $k \ge 1$, as desired.
\end{proof}

==> newcommands.tex <==
\newcommand{\percparam}{\lambda}
\newcommand{\percparamsmall}{\lambda_{s}}
\newcommand{\percparambig}{\lambda_{b}}
\newcommand{\blowupparam}{r}
\newcommand{\boxofpoints}[1]{\fbox{$#1$}}


\newcommand{\LRP}{LRP}
\newcommand{\SFP}{SFP}
\newcommand{\GIRG}{GIRG}

\newcommand{\LRPbig}{LRP_{b}}
\newcommand{\LRPsmall}{LRP_{s}}
\newcommand{\LRPcoupling}{LRP_{c}}

\newcommand{\SFPbig}[1]{SFP_{b}^{#1}}
\newcommand{\SFPsmall}[1]{SFP_{s}^{#1}}
\newcommand{\SFPcoupling}[1]{SFP_{c}^{#1}}


\newcommand{\alphaparam}{\alpha}
\newcommand{\tauparam}{\tau}
\newcommand{\powerlaw}[1]{w_{#1}}
\newcommand{\clow}{c_{\text{low}}}
\newcommand{\cupp}{c_{\text{upp}}}

\newcommand{\probconnection}[1]{1 - e^{-#1|u - v|^{-d\alphaparam}}}
\newcommand{\probnotconnection}[1]{e^{-#1|u - v|^{-d\alphaparam}}}

\newcommand{\graphdist}[2]{\mathcal{D}_{G}(#1, #2)}

